Learning Structured Sparsity in Deep Neural Networks

High demand for computation resources severely hinders deployment of large-scale Deep Neural Networks (DNN) in resource constrained devices. In this work, we propose a Structured Sparsity Learning (SSL) method to regularize the structures (i.e., filters, channels, filter shapes, and layer depth) of DNNs. SSL can: (1) learn a compact structure from a bigger DNN to reduce computation cost; (2) obtain a hardware-friendly structured sparsity of DNN to efficiently accelerate the DNNs evaluation. Experimental results show that SSL achieves on average 5.1x and 3.1x speedups of convolutional layer computation of AlexNet against CPU and GPU, respectively, with off-the-shelf libraries. These speedups are about twice speedups of non-structured sparsity; (3) regularize the DNN structure to improve classification accuracy. The results show that for CIFAR-10, regularization on layer depth can reduce 20 layers of a Deep Residual Network (ResNet) to 18 layers while improve the accuracy from 91.25% to 92.60%, which is still slightly higher than that of original ResNet with 32 layers. For AlexNet, structure regularization by SSL also reduces the error by around ~1%. Open source code is in https://github.com/wenwei202/caffe/tree/scnn

==> tables/alexnet.tex <==
\begin{table}[b]
  \caption{Sparsity and speedup of AlexNet on ILSVRC 2012}
  \label{tab:alexnet}
  \centering
  
  \resizebox{\textwidth}{!}{
  	\begin{tabular}{ccclllllllll}
  		\toprule[0.12 em]
  		\textit{AlexNet}~\# & Method & Top1 err. & Statistics & conv1 & conv2\_1 & conv2\_2 & conv3 & conv4\_1 & conv4\_2 & conv5\_1 & conv5\_2\\

  		\midrule[0.12 em]
  		
  		\multirow{3}{*}{1} & \multirow{3}{*}{$\ell_1$\textsuperscript{\textsection}} & \multirow{3}{*}{44.67\%} & 
  		ES\textsuperscript{\textsterling}  & 67.6\% & 90.2\% & 94.6\% & 97.2\% & 97.8\% & 95.4\% & 95.5\% & 93.2\% \\
  		& & & 
  		CPU $\times$ & 0.80 & 1.76 & 4.06 & 4.84 & 3.46 & 4.20 & 2.39 & 3.13 \\
  		& & & 
  		GPU $\times$ & 0.25 & 0.43 & 0.61 & 1.38 & 1.14 & 0.93 & 1.52 & 1.20 \\
  		\cmidrule{1-12}
  		
  		
  		\multirow{5}{*}{2} & \multirow{5}{*}{SSL\textsuperscript{\textasteriskcentered}} & \multirow{5}{*}{44.66\%} &
  		ES  & 31.6\% & 74.3\% & 91.5\% & 94.2\% & 97.7\% & 93.4\% & 91.4\% & 84.7\% \\
  		& & & 
  		CS\textsuperscript{\textsterling}  & 0.0\% & 51.2\% & 75.2\% & 76.9\% & 90.6\% & 78.8\% & 87.3\% & 74.1\% \\
  		& & & 
  		RS\textsuperscript{\textsterling}  & 9.4\% & 3.9\% & 21.9\% & 40.6\% & 54.2\% & 39.6\% & 0.0\% & 0.0\% \\
  		& & & 
  		CPU $\times$ & 1.05 & 2.14 & 4.59 & 6.27 & 12.58 & 6.87 & 6.16 & 3.69 \\
  		& & & 
  		GPU $\times$ & 1.00 & 1.87 & 2.88 & 4.94 & 4.86 & 3.20 & 3.67 & 2.43 \\
  		\cmidrule[0.12 em]{1-12}
  		
  		\multirow{3}{*}{3} & \multirow{3}{*}{$\ell_1$\textsuperscript{\textsection}} & \multirow{3}{*}{42.51\%} &
  		ES  & 14.7\% & 74.1\% & 78.2\% & 85.3\% & 84.5\% & 78.5\% & 79.4\% & 73.2\% \\
  		& & & 
  		CPU $\times$ & 0.34 & 0.93 & 1.06 & 1.30 & 1.25 & 0.95 & 1.04 & 0.82 \\
  		& & & 
  		GPU $\times$ & 0.08 & 0.16 & 0.18 & 0.42 & 0.32 & 0.28 & 0.29 & 0.34 \\
  		\cmidrule{1-12}
  		
  		\multirow{5}{*}{4} & \multirow{5}{*}{SSL\textsuperscript{\textasteriskcentered}} & \multirow{5}{*}{42.53\%} &
  		ES  & 14.1\% & 51.3\% & 54.9\% & 71.8\% & 77.1\% & 59.7\% & 67.0\% & 48.1\% \\
  		& & & 
  		CS  & 0.00\% & 20.3\% & 21.5\% & 39.7\% & 55.6\% & 23.7\% & 39.8\% & 9.4\% \\
  		& & & 
  		RS  & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% \\
  		& & & 
  		CPU $\times$ & 1.03 & 1.27 & 1.28 & 1.64 & 2.05 & 1.30 & 1.54 & 1.11 \\
  		& & & 
  		GPU $\times$ & 1.00 & 1.24 & 1.26 & 1.63 & 2.14 & 1.29 & 1.61 & 1.11 \\
  		
  		\bottomrule[0.12 em]
  		\multicolumn{11}{l}{\textsuperscript{\textsection} Speedups are implemented by Compressed Sparse Row. \textsuperscript{\textasteriskcentered} Speedups are implemented by concatenation scheme.} \\
  		\multicolumn{11}{l}{\textsuperscript{\textsterling} ES \textendash{} Element Sparsity, CS \textendash{} Column Sparsity, RS \textendash{} Row Sparsity.}
  	\end{tabular}
  }
\end{table}

==> tables/lenet_filter_channel.tex <==
\begin{table}[t]
  \caption{Learning importance of filters and channels in LeNet}
  \label{tab:fc:lenet}
  \centering

  
  %\resizebox{\textwidth}{!}{
  	\begin{tabular}{ccccccc}
  		\toprule
  		LeNet\# & Error & Layer & Filter\# & Channel\# & FLOP & Speedup \\
  		\midrule
  		
  		\multirow{2}{*}{1} & \multirow{2}{*}{0.9\%}  & conv1 & 20 & 1 & 100\% & 1.00$\times$ \\
  		& & conv2 & 50 & 20 & 100\% & 1.00$\times$ \\
  		\cmidrule{1-7}
  		
  		\multirow{2}{*}{2} & \multirow{2}{*}{0.8\%} & conv1 & 5  & 1 & 25\%  & 1.64$\times$ \\
  		& & conv2 & 19 & 4  & 7.6\% & 5.23$\times$ \\
  		\cmidrule{1-7}
  		
  		\multirow{2}{*}{3} & \multirow{2}{*}{1.0\%} & conv1 & 3  & 1 & 15\%  & 1.99$\times$ \\
  		& & conv2 & 12 & 3  & 3.6\% & 7.44$\times$ \\
  		\bottomrule
  	\end{tabular}
  %}
\end{table}

==> tables/lenet_filter_channel_mlp.tex <==
\begin{table}[t]
	
\parbox{.5\textwidth}{
	\caption{Learning importance of filters and channels in LeNet}
	\label{tab:fc:lenet}
	\centering
	
	\resizebox{.5\textwidth}{!}{
	\begin{tabular}{ccccccc}
		\toprule
		LeNet\# & Error & Layer & Filter\# & Channel\# & FLOP & Speedup \\
		\midrule
		
		\multirow{2}{*}{1} & \multirow{2}{*}{0.9\%}  & conv1 & 20 & 1 & 100\% & 1.00$\times$ \\
		& & conv2 & 50 & 20 & 100\% & 1.00$\times$ \\
		\cmidrule{1-7}
		
		\multirow{2}{*}{2} & \multirow{2}{*}{0.8\%} & conv1 & 5  & 1 & 25\%  & 1.64$\times$ \\
		& & conv2 & 19 & 4  & 7.6\% & 5.23$\times$ \\
		\cmidrule{1-7}
		
		\multirow{2}{*}{3} & \multirow{2}{*}{1.0\%} & conv1 & 3  & 1 & 15\%  & 1.99$\times$ \\
		& & conv2 & 12 & 3  & 3.6\% & 7.44$\times$ \\
		\bottomrule
	\end{tabular}
	}
}
\hfill
\parbox{.5\textwidth}{
  \centering
  \caption{Learning the number of neurons in multi-layer perceptron}
  \label{tab:mlp}

  \resizebox{.5\textwidth}{!}{
  	\begin{tabular}{ccccc}
  		\toprule
  		MLP\# & Error & Layer & Neuron\# & FLOP \\
  		\midrule
  		
  		\multirow{3}{*}{1} & \multirow{3}{*}{1.43\%}  & Input & 784 & 100\% \\
  		& & hidden1 & 500 & 100\%  \\
  		& & hidden2 & 300 & 100\%  \\
  		\cmidrule{1-5}
  		
  		\multirow{3}{*}{2} & \multirow{3}{*}{1.34\%}  & Input & 469 & 35.18\% \\
  		& & hidden1 & 294 & 32.54\%  \\
  		& & hidden2 & 166 & 55.33\%  \\
  		\cmidrule{1-5}

  		
  		\multirow{3}{*}{3} & \multirow{3}{*}{1.53\%}  & Input & 434 & 19.26\% \\
  		& & hidden1 & 174 & 9.05\%  \\
  		& & hidden2 & 78 & 26.00\%  \\
  		\bottomrule
  	\end{tabular}
  }
}

  
\end{table}

==> tables/lenet_shape_gemm.tex <==
\begin{table}[t]
  \caption{Results after learning filter shapes in \textit{LeNet}}
  \label{tab:shape:lenet}
  \centering
  \small
  \vspace{-6pt}
  %\resizebox{\textwidth}{!}{
  	\begin{tabular}{cccccccc}
  		\toprule
  		\textit{LeNet} \#& Error & Layer & Filter size \textsuperscript{\textsection} & Channel \# & GEMM & FLOPs & Speedup \\
  		\midrule
  		
  		\multirow{2}{*}{1 (\textit{baseline})} & \multirow{2}{*}{0.9\%}  & conv1 & 25 & 1 & (20, 25)$\times$(25, 576) & 100\% & 1.00$\times$ \\
  		& & conv2 & 500 & 20 & (50, 500)$\times$(500, 64) & 100\% & 1.00$\times$ \\
  		\cmidrule{1-8}
  		
  		\multirow{2}{*}{4} & \multirow{2}{*}{0.8\%}  & conv1 & 21 & 1 & (2, 21)$\times$(21, 576) & 8.4\% & 2.33$\times$ \\
  		& & conv2 & 41 & 2 & (50, 41)$\times$(41, 64) & 8.2\% & 6.93$\times$ \\
  		\cmidrule{1-8}
  		
  		\multirow{2}{*}{5} & \multirow{2}{*}{1.0\%}  & conv1 & 7 & 1 & (1, 7)$\times$(7, 576) & 1.4\% & 5.19$\times$ \\
  		& & conv2 & 14 & 1 & (50, 14)$\times$(14, 64) & 2.8\% & 10.82$\times$ \\
  		\bottomrule
  		\multicolumn{8}{l}{\textsuperscript{\textsection} the size of filter after removing zero shape fibers}
  	\end{tabular}
  %}
\end{table}

==> tables/mlp.tex <==
\begin{table}[t]
  \caption{Learning the number of neurons in multi-layer perceptron}
  \label{tab:mlp}
  \centering

  %\resizebox{\textwidth}{!}{
  	\begin{tabular}{ccccc}
  		\toprule
  		MLP\# & Error & Layer & Neuron\# & FLOP \\
  		\midrule
  		
  		\multirow{3}{*}{1} & \multirow{3}{*}{1.43\%}  & Input & 784 & 100\% \\
  		& & hidden1 & 500 & 100\%  \\
  		& & hidden2 & 300 & 100\%  \\
  		\cmidrule{1-5}
  		
  		\multirow{3}{*}{2} & \multirow{3}{*}{1.34\%}  & Input & 469 & 35.18\% \\
  		& & hidden1 & 294 & 32.54\%  \\
  		& & hidden2 & 166 & 55.33\%  \\
  		\cmidrule{1-5}

  		
  		\multirow{3}{*}{3} & \multirow{3}{*}{1.53\%}  & Input & 434 & 19.26\% \\
  		& & hidden1 & 174 & 9.05\%  \\
  		& & hidden2 & 78 & 26.00\%  \\
  		\bottomrule
  		%\multicolumn{5}{l}{\textsuperscript{\textdagger} footnote}
  	\end{tabular}
  %}
\end{table}

==> tables/mlp_small.tex <==
\begin{table}[b]
  \caption{Learning the number of neurons in multi-layer perceptron}
  \label{tab:mlp}
  \centering
  \small
  \vspace{-6pt}
  %\resizebox{\textwidth}{!}{
  	\begin{tabular}{clll}
  		\toprule
  		\textit{MLP} \# & Error & Neuron \# per layer \textsuperscript{\textsection} & FLOP per layer \textsuperscript{\textsection} \\
  		\midrule
  		
  		1 (\textit{baseline}) & 1.43\%  & 784\textendash500\textendash300\textendash10 & 100\%\textendash100\%\textendash100\% \\
  		%\cmidrule{1-5}
  		
  		2 & 1.34\%  & 469\textendash294\textendash166\textendash10 & 35.18\%\textendash32.54\%\textendash55.33\% \\
  		%\cmidrule{1-5}

  		3 & 1.53\%  & 434\textendash174\textendash78\textendash10 & 19.26\%\textendash9.05\%\textendash26.00\% \\
  		\bottomrule
  		\multicolumn{4}{l}{\textsuperscript{\textsection}In the order of \textit{input layer}\textendash\textit{hidden layer 1}\textendash\textit{hidden layer 2}\textendash\textit{output layer}}
  	\end{tabular}
  %}
\end{table}
